IP over Voice-over-IP for censorship circumvention

Open communication over the Internet poses a serious threat to countries with repressive regimes, leading them to develop and deploy network-based censorship mechanisms within their networks. Existing censorship circumvention systems face different difficulties in providing unobservable communication with their clients; this limits their availability and poses threats to their users. To provide the required unobservability, several recent circumvention systems suggest modifying Internet routers running outside the censored region to intercept and redirect packets to censored destinations. However, these approaches require modifications to ISP networks, and hence requires cooperation from ISP operators and/or network equipment vendors, presenting a substantial deployment challenge. In this report we propose a deployable and unobservable censorship-resistant infrastructure, called FreeWave. FreeWave works by modulating a client's Internet connections into acoustic signals that are carried over VoIP connections. Such VoIP connections are targeted to a server, FreeWave server, that extracts the tunneled traffic of clients and proxies them to the uncensored Internet. The use of actual VoIP connections, as opposed to traffic morphing, allows FreeWave to relay its VoIP connections through oblivious VoIP nodes, hence keeping itself unblockable from censors that perform IP address blocking. Also, the use of end-to-end encryption prevents censors from identifying FreeWave's VoIP connections using packet content filtering technologies, like deep-packet inspection. We prototype the designed FreeWave system over the popular VoIP system of Skype. We show that FreeWave is able to reliably achieve communication bandwidths that are sufficient for web browsing, even when clients are far distanced from the FreeWave server.

==> files/abs.tex <==

\begin{abstract}









Open communication over the Internet poses a serious threat to countries
with repressive
regimes, leading them to develop and deploy network-based censorship
mechanisms within their networks.
Existing censorship circumvention systems face different difficulties in providing 
\textit{unobservable} communication with their clients; this limits their \emph{availability} 
and poses threats to their users.  
To provide the required unobservability, several recent circumvention systems suggest
modifying Internet routers running outside the censored region
to intercept and redirect packets to censored destinations.
However, these approaches require modifications to ISP networks,
and hence requires cooperation from ISP operators and/or
network equipment vendors, presenting a substantial deployment challenge.

In this paper we propose a deployable and unobservable censorship-resistant infrastructure, called \name. 
\name works by modulating a client's Internet connections into acoustic signals that are carried over  VoIP connections. Such VoIP connections are targeted to a server, \name server,  that extracts the tunneled traffic of clients and  proxies them to the uncensored Internet. 
The use of actual VoIP connections, as opposed to traffic morphing, allows \name to relay its VoIP connections through oblivious VoIP nodes, hence keeping itself  unblockable from censors that perform IP address blocking.
Also, the use of end-to-end encryption prevents censors from identifying \name's VoIP connections using packet content filtering technologies, like deep-packet inspection.

We prototype the designed \name system over the popular VoIP system of Skype. We show that \name is able to reliably  achieve communication bandwidths that are sufficient for web browsing, even when clients are far distanced from the \name server.        
 





\end{abstract}


==> files/concl.tex <==
\section{Coclusions}\label{sec:concl}



In this paper, we presented \name, a censorship circumvention system that is highly unblockable by censors. 
\name works by modulating a client's Internet traffic inside the acoustic signals that are carried over VoIP connections. Being modulated into acoustic signals, as well as the use of encryption makes \name's VoIP connections unobservable by a censor. By building a prototype implementation of \name we show that \name can be used to achieve connection bit rates that are suitable for normal web browsing.
   

==> files/discussions.tex <==

\section{Discussions}\label{sec:discussions}
\subsection{Evalution of the design  goals}\label{sec:goals-eval}
In Section~\ref{sec:goals}, we listed several features that we consider in designing an effective circumvention system. Here, we discuss the extent to which our proposed system, \name, achieves such requirements.



\paragraphb{Unblockability:}
In order to use \name, a client only needs to know the VoIP ID of the \name server, i.e., {\tt server-id}, but no other secret/public information like the server's IP address. {\tt server-id} is distributed in a public manner to the users, so we assume that it is also known to censors.  Considering the use of encrypted VoIP connections by \name, this public knowledge of {\tt server-id}  does not allow censors to identify (and block) the VoIP connections to \name server. In addition, a censor will not be able to identify \name's VoIP connections from their IP addresses since, as discussed in Section~\ref{sec:voip}, the encrypted VoIP connections to the \name server are relayed through oblivious, intermediate nodes. For instance, in Skype-based \name the VoIP connections to the \name server are relayed by oblivious Skype super nodes.  Also, \name server  is not mapped to a particular set of super nodes, i.e.,  its VoIP connections are relayed through a varying set of super nodes.
Another point in making \name unblockable is that it does not depend on a particular VoIP system, and can use any VoIP provider for its connections. As a result, in order to block \name, censors will need to block \emph{all} VoIP services, which is very unlikely due to several political and economical considerations.

Note that unblockability is a serious challenge with many existing circumvention systems, as the information advertised for their utilization  can be used by censors to block them. For example, the Tor~\cite{tor} system requires its clients to connect to a public set of its IP addresses, which can be IP-filtered by censors. More recently, Tor has adopted the use of Tor \emph{bridges}~\cite{tor-bridge}, which are volunteer proxies with semi-public IP addresses.  Unfortunately, there are different challenges \cite{Sovran2008,McCoy2011,McLachlan2009a} in distributing the IP addresses of Tor bridges only to real clients, but not to the censors.



\paragraphb{Unobservability:}
The arguments made above for \name's unblockability can also be used to justify its unobservability.  
As mentioned above, even though \name server's VoIP ID ({\tt server-id}) is assumed to be known to censors, the end-to-end encryption of VoIP connections prevents a censor from observing users making VoIP connections to {\tt server-id}. In addition, VoIP relays sitting between \name clients and a \name server, e.g., Skype super nodes, prevent identification of \name connections by matching IP addresses.


\paragraphb{Security:} We devote Section~\ref{sec:security} to discussing the security of \name.


\paragraphb{Deployment feasibility:}
The real-world deployment of \name does not rely on other entities. This is in contrast to some recent designs that need collaboration from third parties for their operation. For instance, Infranet~\cite{infranet} requires support from some web destinations that host the circumvention servers. As another example, several recent systems~\cite{Wustrow2011,Karlin2011,Houmansadr2011a} rely on collaboration from friendly ISPs for their operation.



\paragraphb{Quality of service:}
In Section~\ref{sec:impl}, we discus the connection performance provided by our prototype implementation of \name. Our results show that \name provides reliable connections that are good for normal web browsing. 


%\paragraphb{Ease of use:}\amc{remove?}





\subsection{Security analysis}\label{sec:security}

In this section, we discuss the security of \name clients to threats imposed by different entities.
%Privacy, anonymity and security discussions under different scenarios

%encrypted VoIP,

%p2p VoIP

%centralised VoIP
\subsubsection{Security from censors}

%{\bf Anonymity: }

%{\bf Privacy and confidentiality:}
The end-to-end encryption of VoIP connections protects the confidentiality of the data being sent by \name clients from a monitoring censor, even if the censor is able to identify VoIP connections targeted to \name. Such end-to-end encryption also ensures the web browsing privacy of \name clients.
As mentioned in Section~\ref{sec:voip}, Skype  calls are encrypted end-to-end, and,  SIP-based VoIPs also provide end-to-end encryption using the SRTP protocol.

%{\bf Traffic analysis by the censor:}
Even though \name uses encrypted VoIP connections a censor may still try to identify \name-generated VoIP connections by performing traffic analysis, i.e., by analyzing communication patterns. Since \name makes \emph{real} VoIP connections,  traffic patterns of \name's VoIP connections  will be indistinguishable from those of typical VoIP traffic. In order to better disguise traffic patterns, a \name client can make video calls, instead of voice-only calls, and use the audio channel of the video calls for tunneling \name traffic. This can better hide the traffic pattern of \name VoIP connections, as discussed in  \cite{skypemorph}.
%This is unlike some other circumvention systems that try to foil traffic analysis by shaping their traffic \cite{skypemorph,more}.



\subsubsection{Security from \name servers}

%{\bf Anonymity: }
A \name server only knows the VoIP IDs of its client, but not their IP addresses since the VoIP connections are being relayed through intermediate VoIP nodes, as described before. As a result, unless the VoIP service is colluding  with a \name server,  the \name server will not be able to  link VoIP IDs to IP addresses.

%{\bf Privacy and confidentiality: }
In the basic design of \name mentioned above a  \name server can observe the traffic contents the browsing activity corresponding to a client VoIP ID, since the tunneled traffic is not always encrypted. However, a client can easily ensure security and privacy from the server by using  an extra layer of encryption. For instance, a client can use \name to get connected to an anonymity system like Anonymizer~\cite{anonymizer}, and then use the tunnelled connection with this anonymity system to browse the Internet. This secures this client's traffic from the \name server, as well as makes it confidential. Note that considering the fact that \name clients are always anonymized from \name servers, clients may opt not to use such an additional protection for  low-sensitivity activities like web browsing.


\subsubsection{Security from VoIP providers}

%{\bf Anonymity: }

%{\bf Privacy and confidentiality:}
The VoIP connections between \name clients and servers are encrypted end-to-end; as a result, the VoIP provider will not be able to observe neither the data being communicated, nor the web destinations being browsed through such connections. However, the VoIP service provider is able to identify VoIP IDs that have made VoIP calls to \name server. As a result, in order to ensure its unobservability \name needs to use  VoIP providers that  are not colluding with censors. Note that \name does not rely on a particular VoIP system and any VoIP provider can be used for its operation.



%\amc{talk abut the use of video calls, one way voice, etc.}


==> files/eval.tex <==
\section{Evaluations}\label{sec:eval}


provide results on the capacity of the channel, 
different distances between users, 
the use of different encoders(different rates), 


==> files/impl.tex <==
\section{Implementation and results}\label{sec:impl}

We build a prototype implementation of \name over Skype. 
We use MATLAB7 to build our MoDem component, and we use Virtual Audio Card~\footnote{\url{http://software.muzychenko.net/eng/vac.htm}} as our virtual sound card (VSC) software. We also use the Skype client software provided by Skype Inc.\ as our VoIP client component.     Our MoDem software, as well as the Skype client are set up to use the Virtual Audio Card as their audio interface.  
We build  \name client and a \name server, using the components mentioned above. In order to emulate a real-world experience, i.e., a long distance between \name client and \name server, we connect our \name client to the Internet though a VPN connection. In particular we use the SecurityKISS VPN solution that allows us to pick VPN servers located in different geographical locations around the world. In particular, in our experiments we use VPN servers that are located in Poland and USA. Note that this identifies the location of our \name client, and our \name server is located within  USA (near Indianapolis). 


\paragraphb{MoDem Specifications:} Our evaluations show that the data rates that can be achieved with our system clearly depend on the quality of the Skype connection. The minimum bandwidth required for a voice call is 30 kbps for both upload and download speed, according to Skype. The pulse function of  $p(t)$   is a square-root raised cosine filter with a roll-off factor $0.2$ and a bandwidth  of $1/T$. The carrier frequency $f_C$ is chosen such that the spectrum of the voiceband is always covered. At the receiver the same square-root raised cosine filter is used for low-pass filtering. Our communication system automatically adjusts the symbol constellation size $Q$, the channel coding rate $R_c$ and the symbol period $T$ such that the best possible data rate is achieved. The receiver knows how well the training symbols were received and based on this feedback the transmitter can optimize the data rate. The relationship between the data rate $R$ and the above parameters is
\begin{align}
R = \frac{Q R_c}{T}.
\end{align}
The receiver used in our setup is iterative. The number of iterations needed for convergence depend on the channel condition. The channel condition is typically measured by means of signal to noise power ratio, the SNR. 
Figure \ref{fig:iter} shows the bit error rate (BER) performance of our receiver for given SNR. The plot also compares two different channel codes. A turbo code (precoded) and a regular convolutional code (not precoded). 

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figs/BERvSNR}
\caption{BER versus SNR for \name.}
\label{fig:iter}
\end{figure}

\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Data rate ($R$) & $Q$ & $1/T$ & $R_C$ &  Packet drop rate & Location of client\\\hline
16000 bps & 4 & 8000 kHz & 0.5 & 0.06 & Lodz, Poland\\\hline
19200 bps & 4 & 9600 kHz & 0.5 & 0.01 & Chicago, IL\\\hline
\end{tabular}
\caption{Evaluation results of \name. }
\label{tab:res}
\end{table*}

Our results are summarized in table \ref{tab:res}. The table lists the best compromise between the   data rates and the packet drop rate,  for various destinations. As can be seen, for our \name server being located in midwest (near Indianapolis)  a \name client can get a reliable  connection with  a bit rate of 19.2 kbps , while a user in Poland achieves a connection bit rate of 16 kbps.  These bit rates are convenient for regular web browsing, which is the main intent of censored users. Also, note that while \name provides a  fairly low bit-rate, as compared to other circumvention systems, its connections is highly unblockable, as discussed throughout this paper.  










==> files/intro.tex <==
\section{Introduction}\label{sec:intro}




% censorship problem is serrious
The Internet is playing an ever increasing role in connecting people from across the world, facilitating the free
circulation of speech, ideas and information. This poses a serious threat to the benefits and,  even,  the existence
of repressive regimes as it elevates their citizens' awareness and provides them a powerful media to
arrange coordinated opposition movements. The recent unrest in the Middle East indicates the very strong power of the Internet in arranging nation-wide protests that, in several cases, has resulted in revolutionizing or even overthrowing repressive regimes.
To response to such threats, repressive regimes make use of different technologies to restrict and monitor their citizens' access to the Internet, known as \emph{Internet censorship}. Censorship devices, called \emph{censors}, leverage techniques \cite{gifc:07, Leberknight2010} ranging from simple IP address blocking and DNS hijacking, to the more complicated and resource-intensive deep packet inspection (DPI) in order to enforce their restrictions and monitoring. Citizens identified  non-complying with such restrictions can face consequences ranging from Internet service disruption to life-threatening punishments.


% existing circumnvetntion approaches

To help the censored users  gain open access to the Internet different systems and technologies have been designed and developed, generally referred to as  \emph{censorship circumvention} tools. These systems are  composed of computer and networking technologies and allow Internet users to evade monitoring, blocking, and tracing of their activities over the Internet.
Early circumvention systems work by \emph{proxy}ing the Internet traffic of their users to censored Internet destinations,  foiling  IP-address blocking and DNS hijacking performed by censors. Examples of such systems are DynaWeb~\cite{dynaweb}, Anonymizer~\cite{anonymizer}, and Freenet~\cite{freenet}. The use of  advanced content filtering technologies~\cite{gifc:07, Leberknight2010}, i.e., deep packet inspection,  by censors renders the use of simple proxies ineffective for censorship evasion. This resulted in  the advent of more sophisticated circumvention systems like Ultrasurf~\cite{ultrasurf} and Psiphon~\cite{psiphon} that try to confuse  content filtering tools by obfuscating their design and/or traffic patterns. Such obfuscation does not provide strong security promises for users, as investigated in recent study \cite{ultrasurf-analysis}.  More recently, several circumvention systems are designed that work by hiding the circumvented traffic in regular Internet traffic \cite{infranet, collage, Wustrow2011, Houmansadr2011a}. In addition to special-purpose circumvention systems, \emph{anonymity systems} are also often used for censorship circumvention. Anonymity systems aim in  hiding the browsing activity of users from other parties, a objective in common with circumvention systems. For instance, the Tor~\cite{tor} anonymity system has recently adopted the use of semi-public nodes, known as Tor bridges~\cite{tor-bridge}, that help censored users to gain unrestricted access to the Internet anonymously. Through the rest of this paper, by circumvention systems we consider both circumvention-centric systems and the anonymity systems adopted to evade censorship.

% limitation of current approaches

While these circumvention systems have long been used by many users from across the world  they suffer from several important shortcomings.
The biggest threat to existing circumvention systems is their weak \emph{availability} to  users, i.e., they lack \emph{unblockability}. Censors proactively look for   services that help  with censorship circumvention and either disrupt their operation, or block their citizens from accessing them.
In particular, censors rigorously look for  IP addresses belonging to circumvention technologies (e.g., HTTP/SOCKS proxies) and add them to IP blacklists maintained by their censoring firewalls \cite{italy-block, gifc:07}.
 As a result, citizens under repressive regimes commonly find it  difficult to access  operating  circumvention systems. For instance the popular Tor system has frequently been/is blocked by censorship regimes \cite{tor-blocked,china-tor}, making it unavailable to users in certain countries.
To improve their availability, circumvention systems have taken different approaches to make their connections \emph{unobservable} to censors, hence unblockable.
The Tor system, for instance, has deployed Tor bridges~\cite{tor-bridge} that are volunteer proxies  whose IP addresses are distributed among Tor users in a selective manner. This makes Tor bridges less prone to be identified by censors, as compared to Tor entry nodes, however  there are several challenges in distributing their IP addresses among users \cite{McCoy2011,McLachlan2009a}. Other systems \cite{infranet, collage} try to provide unobservability (hence availability) by pre-sharing some secret information with their users. This, however, is neither scalable, nor effective, as it is challenging to share secrets with a large number of real users, while keeping them secret from  censors \cite{Feamster03,springerlink:10.1007/978-3-642-13122-6_29,Sovran2008}. More recently, several systems are proposed that rely on support from third-parties for their operation. For instance Telex~\cite{Wustrow2011} and Cirripede~\cite{Houmansadr2011a} work by concealing the circumvented traffic inside regular traffic thanks to some friendly ISPs that deflect/manipulate their intercepted traffic. The real-world deployment of such circumvention systems requires collaboration of several trusted ISPs that make software and/or hardware modifications to their infrastructure; this does not seem to be realized in short-time until there are enough financial motives for the ISPs.


% our approach, then the key features of our system

In this paper, we design \name, a censorship circumvention system that is highly unblockable\footnote{We use terms \emph{unblockability} and \emph{availability} interchangeably.}. The main idea of \name, as shown in Figure~\ref{fig:main}, is to tunnel Internet traffic inside non-blocked VoIP communications by  modulating them into acoustic signals that are carried over VoIP connections.
For a censored user to use \name for circumvention, she needs to setup a  VoIP account with a public VoIP provider,  and also to install \name's client software on her machine.
Part of the \name system is a \name server that listens on several publicly advertised VoIP IDs for connections from its clients.  To make a \name connection, a user's \name client software makes VoIP connections to  \name server's VoIP IDs. The client and server, then, tunnel the circumvented Internet traffic inside the established VoIP connections, by modulating network packets  into  acoustic signals carried by the established VoIP connections.
%Being modulated into real acoustic signals, also the use of encryption and coding algorithms, provides high unobservability  for \name's operation, as discussed in the following.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/main-scheme}
\caption{The main architecture of \name.}
\label{fig:main}
\end{figure*}

We claim that \name provides strong unblockability promises since its unblockability is tied to the availability of VoIP communications. VoIP constitutes an important part of today's Internet communications \cite{voip-stat,voip-penetration,voip-importance}, hence censors are not willing to block \emph{all} VoIP communications due to several financial and political reasons.
A recent  report \cite{voip-penetration} shows that about one-third of U.S.\ businesses use VoIP solutions to reduce their telecommunications expenses, and the report predicts the  VoIP penetration   to reach 79\% by 2013, a 50\% increase compared to 2009.   \name's availability is tied to the availability of VoIP service: as the operation of \name is not bound to a specific VoIP provider,  in order to block \name a censor needs to block \emph{all} VoIP service providers.
We also claim that a censor can not distinguish \name-related VoIP traffic from regular VoIP traffic:  the modulation of circumvented traffic inside real acoustic signals, as well as the use of encryption and coding algorithms makes \name's VoIP connections \emph{unobservable} to censors. In addition, the way \name server is connected to the Internet results in getting \name's VoIP connections to be \emph{relayed} by various \emph{oblivious VoIP peers}, preventing a censor from blocking/identifying \name's VoIP connections by matching IP addresses (see Figure~\ref{fig:main}). 
In fact, this is the key feature  distinguishing \name from similar circumvention systems that work by morphing  circumvented traffic to look like other protocols. For instance, SkypeMorph~\cite{skypemorph} suggests to morph (i.e., shape) a Tor client's traffic to a Tor bridge to look like an encrypted  Skype connection, in order to prevent a censor from identifying the connection as a Tor connection and, hence, detecting the IP address of the morphing Tor bridge. This, however, does not mitigate the big issue of distributing bridge IP address (and Skype IDs for SkypeMorph), so censors can eventually identify IP addresses belonging to the morphing Tor bridges (e.g., by pretending to be real clients), hence block the bridges and/or punish the identified clients. In \name, however, the VoIP connections carrying circumvented traffic are established between clients and some oblivious VoIP peers, so even a censor's knowledge of \name server's IP address can not help him in identifying/blocking \name's VoIP connections (this is in contrast to SkypeMorph where morphed VoIP connections are between clients and the Tor bridges). 



%\name's unobservability, as thoroughly discussed in the paper, provides high availability promises for \name.


% mention how impleemntaed and some resaults

We implement a prototype of \name system over Skype and measure its performance. Our evaluations show that \name provides  connection bit rates that are convenient for regular web browsing. We also validate that \name can be used by clients that are geographically far away from the \name server, with a reasonably lower connection throughput. 

% roadmap
The rest of this paper is organized as follows; in Section~\ref{sec:related} we review related research. In Section~\ref{sec:prelim} we review our threat model and the goals in designing our circumvention system. We describe the design of our proposed circumvention system, \name, in Section~\ref{sec:scheme}, and Section~\ref{sec:detail} discusses our design details. In Section~\ref{sec:discussions}, we discuss the features of our designed circumvention system. Section~\ref{sec:modem} describes the \name's MoDem block, an essential component of \name that modulates Internet traffic into acoustic signals. We describe our prototype implementation of \name in Section~\ref{sec:impl},  along with the evaluation results. Finally, the paper is concluded in Section~\ref{sec:concl}. 





==> files/modem.tex <==
\section{\name MoDem}\label{sec:modem}

The MoDem component  is an essential component of both \name client and \name server, which translates Internet traffic into acoustic signals and vice versa. MoDem consists of a transmitter and a receiver. MoDem's transmitter modulates data (IP bits) into acoustic signals, and MoDem's receiver demodulates data from a received acoustic signal. In the following, we describe the design of  MoDem's transmitter and receiver. 

\subsection{Transmitter description}


The transmitter structure considered here is based on bit-interleaved coded modulation (BICM). First, the information bits $\{ a_i \}$ are encoded by a rate $R_c$ channel encoder, producing the coded bit sequence $\{ b_i \}$. The sequence $\{ b_i \}$ is permuted using a random interleaver and the resulting sequence is then partitioned into length $Q$ subsequences $\boldsymbol{c}_n = [ c_n^1, \ldots, c_n^Q \}$. Each such subsequence is finally mapped to a $2^Q$-ary quadrature amplitude modulation (QAM) symbol. 

Data transmission is carried out frame-by-frame. As shown in Figure \ref{fig:data_SI}, 
a frame consists of $T$ sets of the training symbols followed by the data symbols. A block of known preamble symbols as well as a block of signal symbols are inserted in front of every frame. The preamble symbols are needed for synchronization and receiver initialization purposes. The signal symbols tell the receiver what modulation and coding was used for the data symbols. The training symbols are needed to adapt the equalizer to the time-varying channel.  We enumerate the symbols in this frame by $x_n$.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/data_SI}
\caption{Frame structure}
\label{fig:data_SI}
\end{figure*}

The symbol sequence $x_n$ is mapped to a waveform $x(t): \mathbb{R} \to \mathbb{C}$
\begin{align}
x(t) = \sum_{l} x_l p(t-lT)
\end{align}
by use of a basic pulse $p(t)$ time shifted by multiples of the symbol
period $T$. This signal is then modulated to passband 
\begin{align}
x_{PB}(t) = 2 \Re \{ x(t)e^{2 \pi i f_C t}  \}
\end{align}
at carrier frequency $f_C$ and sent over the Skype channel.

\subsection{Receiver description}

We assume the passband channel effect to be linear. An equivalent baseband channel representation is obtained by demodulating and low-pass filtering the received signal $r(t)$. After synchronization and symbol-spaced sampling, we obtain the equivalent discrete baseband channel observations $r_n$.
\begin{align}
r_n = \sum_{k = -K_f}^{K_p} h_{n,k} x_{n-k} + w_n
\end{align}
where $n$ and $k$ are time and delay indices, respectively and $w_n$ is a complex white Gaussian noise process. The channel length is assumed to be at most $K_f + K_p + 1$, where $K_f$ is the length of the precursor and $K_p$ is that of the postcursor response. We explicitly allow for the channel the gains $h_{n,k}$ to change in time $n$.

A block diagram of the used Turbo Equalizer system is shown in Figure \ref{fig:turboEqualizer}. 
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/turboEqualizer}
\caption{Block diagram of the receiver architecture. $\Pi$ and $\Pi^{-1}$ denote interleaving and deinterleaving operations, respectively.}
\label{fig:turboEqualizer}
\end{figure*}
The equalizer produces extrinsic log-likelihood ratios (LLRs) on the coded bits using the received vector $y_n$ and the a priori LLRs on them \cite{Laot01}. Specifically, the extrinsic LLR $L_{\text{ext}}(c_n^q)$ can be obtained from $L_{\text{ext}}(c_n^q) =   L_{\text{post}}(c_n^q) - L_{\text{pri}}(c_n^q)$, where $L_{\text{pri}}(c_n^q)$ is the \emph{a priori} LLR defined as  $L_{\text{pri}}(c_n^q) = \ln Pr(c_n^q = 1) - \ln Pr(c_n^q = 0)$ and 
$L_{\text{post}}(c_n^q)$ is the a posteriori LLR defined as $L_{\text{post}}(c_n^q)  = \ln Pr(c_n^q = 1| \text{observation}) - \ln Pr(c_n^q = 0| \text{observation})$.
Note that the observation can be any function of $y_n$ and the \emph{a priori} LLRs are obtained from the channel decoder. The extrinsic LLRs produced in the equalizer are delivered to the channel decoder through the deinterleaver. They are used as \emph{a priori} LLRs to produce the additional extrinsic LLRs in the channel decoder. Finally, the extrinsic LLRs obtained by the channel decoder are fed back to the equalizer to aid the equalization task. These steps complete one cycle of turbo iteration and are repeated until a suitably chosen convergence criterion is achieved.



==> files/prelim.tex <==


\section{Preliminaries}\label{sec:prelim}

\subsection{Threat model}

We assume that a \name user, namely \name client, is connecting to the Internet through a censoring ISP, i.e., an ISP that is controlled and regulated by a censorship authority. Based on the regulations of the censoring ISP, its users are not allowed to connect to certain Internet destinations, called the \emph{censored destinations}.
The users are also prohibited from using censorship circumvention technologies that would help them to evade the censoring regulations.
The censoring ISP uses a set of advanced technologies to enforce its censoring regulations, including IP address blocking, DNS hijacking, and deep packet inspection. The censoring ISP also monitors its users' network traffic to identify and block any usage of censorship circumvention tools; traffic analysis can be used by the censor as a powerful technique for this purpose.

We assume that the censoring ISP enforces its regulations  such that it does not compromise the \emph{usability} of the Internet, due to different political and economical reasons. In other words, the  enforced censorship does not disable/disrupt key services of the Internet. In particular, we consider VoIP as a key Internet service in today's Internet \cite{voip-importance,voip-stat,voip-importance-business}, and we assume that, even though a censor may block certain VoIP providers, it will not  block \emph{all} VoIP services.
VoIP constitutes a key part in the design of \name. 



\subsection{System goals}\label{sec:goals}

We consider the following as the key features in designing and evaluating a censorship circumvention system.
Later in Section~\ref{sec:goals-eval}, we discuss these features for the \name circumvention system proposed in the consequent sections and compare \name with related work.


\paragraphb{Unblockability:}
The main goal of a censorship circumvention system is to help censored users gain access to censored Internet destinations. As a result, the most trivial property of a circumvention system is being accessible by  censored users, i.e., it should not be unblockable by censors.


\paragraphb{Unobservability:}
 Unobservability is to hide  users' utilization of a circumvention system from censorship authorities, which is a challenging feature to achieve due to the recent advances in censorship technologies \cite{gifc:07}. The importance of unobservability is two-fold; first, an observable circumvention can jeopardize the  safety of a user who has been caught by the censor while using the circumvention system; and,  second, a weak  unobservability commonly results in a weak unblockability, as  it allows censors to more easily identify, hence block, traffic generated by the circumvention system.

\paragraphb{Security:} 
Several security considerations should be made once analyzing a circumvention system. These considerations include users' anonymity, security and privacy from different entities including the censors, the utilized circumvention system,  and other third-parties. 


\paragraphb{Deployment feasibility:}
An important feature of a circumvention system is the amount of resources (e.g., hardware, network bandwidth, etc.) required for it to be deployed in real-world.  A circumvention system is also desired to have few dependencies on other systems and entities in order to make it more reliable, secure, and cost-effective.


\paragraphb{Quality of service:}
A key feature in making a circumvention system popular in practice is the quality of service provided by it in establishing circumvented connections. Two important factors are the connection bandwidth, and the browsing latency.

\if 0
\paragraphb{Ease of use:}\amc{remove?}
For a circumvention system to be effective, it should be usable by a wide range of users with various technical expertise.  Ideally, a circumvention system should work by providing a user with a client software that the user installs and configures on her machine, which allows the user to use the system for a long time without the need for frequent re-configurations/re-installations.
\fi



==> files/related.tex <==
\section{Related work}\label{sec:related}


Since the epoch  of Internet censorship, different entities have designed and built systems to combat censorship.
This has resulted  in an arms-race between censors and circumvention systems, a game with no ultimate winner as of now.
Early circumventions systems are based on setting up a \emph{proxy}~\cite{RFC3143} server outside the censorship territories, trying to evade the
simple IP address blocking and DNS hijacking techniques enforced by pioneer censorship systems. Examples of such proxy-based circumvention tools are DynaWeb~\cite{dynaweb}, Anonymizer~\cite{anonymizer}, and Freenet~\cite{freenet}.

Proxy-based circumvention tools lost their capabilities with the advent of more sophisticated censorship technologies, like deep-packet inspection~\cite{gifc:07, Leberknight2010}. Deep-packet inspection analyzes packet contents looking for patterns indicating the circumvention of the enforced censorship.
This has pushed the circumvention tools to correspondingly sophisticate their techniques in order to remain available to users.
In particular, several circumvention system base their availability on being unobservable from censors.
Infranet~\cite{infranet}, for example,  works by sharing  some secret information with its clients, which are then used by the clients to establish unobservable connections with Infranet servers. Collage~\cite{collage} is another system that, similarly, bases its unobservability on sharing secrets with its clients. More specifically, a Collage client and the Collage server secretly agree on some user-generated content sharing websites, e.g., flickr.com, and use steganography to communicate through these websites. The main challenge for these systems is to share secret information with a large set of users such that censors do not get hands on the shared secrets; this is a challenging problem to solve as discussed in several research \cite{Feamster03,Sovran2008,springerlink:10.1007/978-3-642-13122-6_29}. Sharing secret information with users has also been adopted by the popular Tor anonymity network \cite{tor} to help with censorship circumvention. The secret information here are the IP address of several volunteer nodes, Tor bridges~\cite{tor-bridge}, that proxy the connections of Tor clients to the Tor network. This suffers from the same limitation as
censors can pretend to be real Tor users and  gradually identify a large fraction of Tor bridges \cite{McLachlan2009a,McCoy2011}.

More recently, several research propose to build circumvention  into the Internet infrastructure \cite{Karlin2011, Wustrow2011,Houmansadr2011a}.
Being built into the Internet infrastructure makes such circumvention highly unobservable: a client's covert communication with a censored destination appears to the censor to be a benign traffic with a non-prohibited destination. Telex~\cite{Wustrow2011}, Cirripede~\cite{Houmansadr2011a} and Decoy Routing \cite{Karlin2011} are example designs using such infrastructure-embedded approach.  Decoy Routing  needs to share secrets with its clients using out-of-band channels, whereas Telex and Cirripede share the secret information needed to initialize their connections using covert channels inside Internet traffic. Cirripede uses an additional client registration stage that provides some advantages and limitations as compared to Telex and Decoy routing systems. Even though these systems are a large step forward in providing unobservable censorship circumvention their practical deployment is not trivial as they need to be deployed by a number of real-world ISPs that will make software/hardware modifications to their network infrastructures, something that needs enough financial motivations for ISPs to have them deploy it.

Another research trend uses traffic obfuscation as a method to make circumvented traffic unobservable. Appelbaum et al.\ propose a platform that allows one to build protocol-level obfuscation plugins for Tor, called \emph{pluggable transports}~\cite{pluggable-transport}. These plugins obfuscate a Tor client's traffic to Tor bridges by hiding it into another protocol that is allowed by censors. There are two pluggable transports available; obfsproxy~\cite{obfsproxy} obfuscates Tor traffic by passing it through a stream cipher. Mohajeri et al.\ \cite{skypemorph} show that obfsproxy generates traffic patterns that are detectable by powerful censors. They, consequently, propose SkypeMorph \cite{skypemorph} that morphs a Tor client's traffic into Skype video calls, in order to make it undetectable by deep-packet inspection. We argue that even though this prevents a censor from detecting Tor bridges through traffic analysis, the censors can still pretend to be real Tor users and gradually gain the IP addresses of Tor bridges, hence blocking their connections. The authors of SkypeMorph propose frequent change of the detected IP addresses, as well as the detected Skype IDs in response to this. As another possible issue, in SkypeMorph clients need to send key initialization information to tor bridges through Skype text messages. As such messages have a known format they can be detected and blocked by Skype; in particular, since 2007 Skype provides a special version of its client software to Chinese users that monitors and blocks the text messages sent by Chinese users \cite{skype-monitor-china1,skype-monitor-china2,skype-monitor-china3,skype-monitor-china4}.      
CensorSpoofer~\cite{censorspoofer} is another recent research that aims in  providing  unobservable circumvention by morphing circumvented traffic into spoofed VoIP connections. 
A common security concern with morphing approaches is that they do not provide a provable undistinguishability between a morphed traffic and the regular traffic; this may result in finding effective statistical tests, in the future, that are able to detect currently-undetectable morphing techniques, e.g., \cite{skypemorph} mentions the possibility of detecting  Traffic Morphing \cite{Wright2009} by analyzing inter-packet delays.
As another similar circumvention system, TranSteg~\cite{transteg} re-encodes the call stream in a VoIP connection using a different codec in order to free a  portion of VoIP packet payloads, which are then used to send a low-bandwidth circumvented traffic. 


%Several research consider using VoIP services for censorship circumvention by replacing the packet payloads of VoIP traffic with that of circumvented data.
%This had two main drawbacks: one it is detectable by traffic analysis, or by an insider in the voip network , also, proprietary voip systems can block this by adding some integrity check to their software client, e.g., Skype added some capabilities to filter messages in Skype communications in China as of 2007. (ref in wiki)


%\cite{Cao2009}





==> files/scheme.tex <==
\section{\name scheme}\label{sec:scheme}

In this section, we describe the design of \name censorship circumvention.  Figure~\ref{fig:main} shows the main architecture of \name.  
In order to get connected through \name, a user installs a \emph{\name client} on her machine, which can be obtained from an out-of-band channel, similar to other circumvention systems. The user sets up the installed \name client by entering her own VoIP ID and also the publicly known VoIP ID of \name server. Once the \name client starts up, it makes a VoIP audio/video call to \name server's VoIP ID. As discussed in Section~\ref{sec:voip}, the \name server is configured in a way that VoIP connections initiated by clients are relayed through various \emph{oblivious VoIP peer}s, e.g., Skype supernodes; this is a key security feature of \name as it prevents a censor from blocking \name's VoIP connections using IP address blocking. Also, since \name's VoIP connections are end-to-end encrypted, a censor will not be able to identify \name's VoIP connections by analyzing traffic contents, e.g., by looking for the VoIP IDs. Using the established VoIP connection, a \name client circumvents censorship by modulating  its user's Internet traffic into acoustic signals that are carried over by such VoIP  connections. \name server demodulates a client's Internet traffic from the received acoustic signals, and proxies the demodulated traffic to the requested Internet destinations.


Next, we introduce the main components used in \name and, then, describe how these components are used in the design of \name's client and server.







\subsection{Components of \name}\label{sec:comp}
In this section, we introduce the main elements used in the design of  \name client and server software. The first three components are used by both \name client and \name server, while the fourth element is only used by \name server.

\paragraphb{VoIP client} A Voice-over-IP (VoIP) client software that allows VoIP users to connect to one (or more) specific VoIP service(s). In Section~\ref{sec:voip}, we discuss the choices of the VoIP service being used by \name.

\paragraphb{Virtual sound card (VSC)} A virtual sound card is a software application that uses a physical sound card installed on a machine to generate one (or more) isolated, virtual sound card interfaces on that machine. A virtual sound card interface can be used by any application running on the host machine exactly the same way a physical sound card is utilized. Also, the audio captured or played by a virtual sound card does not interfere with that of other physical/virtual sound interfaces installed on the same machine. We use virtual sound cards in the design of \name to isolate the audio signals generated by \name from the audio corresponding to other applications.

\paragraphb{MoDem} \name client and server software  use a modulator/demodular (MoDem) application that translates network traffic into acoustic signals and vice versa. This allows \name to tunnel the network traffic of its clients over VoIP connections by modulating them into acoustic signals. We provide a detailed description of the design of our MoDem in Section~\ref{sec:modem}.

\paragraphb{Proxy} \name server uses an ordinary proxy server application that proxies  the network traffic of \name clients, received over VoIP connections, to their final Internet destinations. 
Two popular choices for \name's proxy are the HTTP proxy \cite{RFC2616} and the SOCKS proxy \cite{RFC1928} protocols; a SOCKS proxy supports proxying of a  wide range of IP protocols, while an HTTP proxy only supports proxying of HTTP/HTTPS traffic, but it can perform HTTP-layer optimizations like pre-fetching of web contents. Several proxy solutions support both  protocols.    

%In Section~\ref{sec:proxy} we discuss the choice of our network proxy.

\subsection{Client design}\label{sec:client}

The \name client software, installed by a \name user, is consisted of the three main components listed above: a VoIP client application, a virtual sound card (VSC), and  the MoDem  application.
Figure~\ref{fig:client} shows the block diagram of the \name client design. MoDem transforms the data of the network connections sent by the web browser into acoustic signals and sends them over to the VSC component. The \name MoDem also listens on the VSC sound card to receive specially formatted acoustic signals that carry modulated Internet traffic; MoDem extracts the modulated Internet traffic from such acoustic signals and sends them to the web browser. In fact, client's web browser uses the MoDem component as a web proxy, i.e., the listening port of MoDem is entered in the HTTP/SOCKS proxy settings of the browser.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/client}
\caption{The main components of \name client.}
\label{fig:client}
\end{figure*}

The VSC sound card acts as a bridge between MoDem and the VoIP client component, i.e., it transfers audio signals between them. More specifically,
the VoIP client is set up to use the VSC sound card as its \emph{speaker} and \emph{microphone} devices (VoIP applications allow a user to specify the (physical/virtual) sound cards to be used with them). This provides MoDem and the VoIP client to exchange audio signals that contain the modulated network traffic, isolated from the audio generated/recorded by other applications on the client machine.

For the \name client to connect to a particular \name server it \emph{only} needs to know the VoIP ID belonging to that \name server, but not the IP address of the \name server. Every time the user starts up the \name client application on her machine the VoIP application of \name client initiates an audio/video VoIP call to the known VoIP ID of the \name server.


\subsection{Server design}\label{sec:server}

Figure~\ref{fig:server} shows the design of \name server, which consists of four main elements.
\name server uses a VoIP client application to connect with its clients through VoIP connections. \name server chooses one or more VoIP IDs, which are provided to its clients, e.g., through public advertisement. 
%In Section~\ref{sec:voip}, we elaborate on the selection of VoIP IDs by the \name server.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figs/server}
\caption{The main components of \name server.}
\label{fig:server}
\end{figure*}

The VOIP client of \name server uses one (or more) virtual sound cards (VSC) as its \emph{speaker} and \emph{microphone} devices. The number of VSCs used by the server depends on the deployment scenario, as discussed in Section~\ref{sec:deployment}. The VSC(s) are also being used by a  MoDem component, that transforms acoustic signals into network traffic and vice versa. More specifically,  MoDem extracts the Internet traffic modulated by \name clients into audio signals from VoIP connections and forwards them to the last element of the \name server, \name \emph{proxy}. The MoDem also modulates Internet traffic received from the proxy component into acoustic signals and sends them to the VoIP client software through the VSC interface.
The \name proxy is a regular network proxy, e.g., an HTTP proxy, that is used by \name server to connect \name clients to the Internet in an unrestricted manner. As mentioned above in Section~\ref{sec:client}, the web browser of a \name client targets its traffic to a network proxy; such proxied traffic is received by \name server's proxy server (through the VoIP connections, as described) and is processed as required.






\section{Other design details}\label{sec:detail}


\subsection{Deployment scenarios}\label{sec:deployment}

The \name system proposed in this paper can be deployed by  "good" entities that run   \name servers to help  censored users  gain an uncensored access to the Internet. We consider the following scenarios for a real-world deployment of \name. In Section~\ref{sec:security}, we discuss the security considerations for each of these scenarios.

\begin{itemize}
\item{Personal deployment:} A   person having an uncensored access to the Internet can set up a personal \name server on her personal machine, trying to \emph{anonymously} help censored users evade censorship. Such a person can, then,  advertise her VoIP ID (associated with her \name server) publicly (e.g., through social networks) and anyone learning this ID would be able to connect to the Internet by running a \name client software. To save her bandwidth, such a person can configure its \name server to enforce restrictions on the quality of service provided to clients.

\item{Central VoIP-center:} \name service can be deployed and maintained by a central authority, e.g., a for-profit or non-profit organization. The deploying organization can build and run \name servers that are a able to serve a large number of \name clients. To be able to support  large numbers of clients, the used \name servers should deploy several physical/virtual sound cards.  Also, by generating VoIP IDs on several, different VoIP service providers such central \name system will be able to service \name clients with different VoIP preferences. Such a central deployment of \name can operate for commercial profit, e.g., by charging clients for using the system, or can be established as a non-profit systems, e.g., being funded by NGOs or pro-freedom governments.

\item{Central phone-center:} As an alternative approach, \name can be deployed using an automated telephone center. More specifically, instead of VoIP IDs, the \name server will publicize several phone numbers, which are used by clients to connect to the \name server. \name users need to use the exact same \name client software, except that instead of making VoIP calls to \name server's VoIP IDs they will make VoIP calls to \name server's phone numbers. Compared to the "central VoIP-center" approach, this has the big advantage that clients can arbitrarily choose any VoIP service provider for the client software, while in the "central service" design users need to choose from the VoIP systems supported by \name server (though a powerful \name server can support many VoIP systems).

 
\item{Distributed service:} \name service can also be deployed in a distributed architecture, similar to that of the popular  anonymity network of Tor~\cite{tor}. More specifically, \name server can be consisted of a number of volunteer computers that run instances of \name server software on their machines. A central authority can manage the addition of new volunteer nodes to the system and also the advertisement (or distribution) of their VoIP IDs to the clients.



\end{itemize}


\subsection{The choice of  VoIP system}\label{sec:voip}

There are numerous freeware and paid \emph{VoIP service provider}s that can be utilized by the \name system, e.g., Skype\footnote{\url{http://www.skype.com}}, Vonage\footnote{\url{http://www.vonage.com}}, iCal\footnote{\url{http://www.icall.com/}},  etc. Each VoIP service provider provides an application software for its clients; also, there are software that support connection to different VoIP providers, e.g., PhonerLite\footnote{\url{http://www.phonerlite.de/index_en.htm}}. In this section, we mention possible VoIP service provider candidates to be used by \name.

\subsubsection{Skype}
Skype is a peer-to-peer VoIP system that provides voice calls, instant messaging, and video calls to its clients over the Internet.
Skype is one of the most popular VoIP service providers with over 663 million users\footnote{\url{http://www.telecompaper.com/news/skype-grows-fy-revenues-20-reaches-663-mln-users}} as of September 2011.

Skype uses an undisclosed proprietary design, which has been analyzed in several research~\cite{Baset2006,Guha2006,Xie2007}. These studies find that Skype uses a  peer-to-peer overlay network with the Skype users as its nodes.  There are two types of nodes on Skype: \emph{ordinary nodes}, and \emph{super nodes (SN)}. Any Skype client with  a public IP address, having sufficient CPU, memory, and network bandwidth is considered a super nodes, and all the other nodes are considered as ordinary nodes. In addition, Skype uses a central \emph{login server} that keeps users' login credentials and is used by Skype users to register into Skype's overlay network. Apart from the login server all  Skype communications work in a peer-to-peer manner, including the user search queries and online/offline user information.

A key feature that makes Skype an ideal choice for \name is its peer-to-peer network. In particular, a VoIP connection made towards an ordinary node in Skype gets relayed by at least one oblivious Skype super node \cite{Baset2006,Guha2006}. 
More specifically, each ordinary node maintains a \emph{host cache (HC)} table that keeps a list of reachable super nodes, which are used by the ordinary node to make  Skype connections.  
We use this feature to protect \name from being blocked by censors: by having our \name server to act as an ordinary node the VoIP connections from \name clients to the \name server will be relayed by alternative super nodes, hence censors will not be able to enforce IP address blocking. We discuss this further in Section~\ref{sec:security}. Note that a \name server can have its VoIP connections be relayed by arbitrarily various super nodes by frequently \emph{flush}ing its HC table  \cite{Baset2006}. 

Based on the criteria mentioned for a  super node, an easy way to be considered an ordinary node by Skype is to sit behind NAT or a firewall~\cite{Guha2006} (since a super node must have a static public IP address).
As a result, in order to have a \name server to be considered as a Skype ordinary node, it can simply be protected by a firewall or can be put behind a NAT with dynamic address allocations. 
As another interesting feature for \name,  all Skype connections are secured by end-to-end encryption~\cite{Baset2006,Guha2006}.



%another reference : Sliver needle in the skype

\cut{
Trafﬁc passes along the
tunnel in ﬁxed-size cells. Each cell is 512 bytes, and consists
of a header and a payload
}
% say "sotware client"


\subsubsection{SIP-based VoIP}
Session initiation protocol~\cite{RFC3261} (SIP) is a light-wight,  popular signaling protocol and is widely used by VoIP providers, e.g., SFLphone\footnote{\url{http://sflphone.org/}}, Zfone\footnote{\url{http://zfoneproject.com/}}, and Blink\footnote{\url{http://icanblink.com/}}, to establish calls between  clients. A SIP-based VoIP system consists of three main elements~\cite{RFC3261}: 1) \emph{user agents} that try to establish SIP connections on behalf of users, 2) a \emph{location service} that is a database keeping information about the users, and 3) a number of \emph{servers} that help users in establishing SIP connections. In particular, there are two types of SIP servers; \emph{registrar} servers receive registration requests sent by  user agents and update the location service database. The second type of SIP servers are the \emph{proxy} servers that receive SIP requests from user agents and other SIP proxies and help in establishing the SIP connections.

Once a SIP connection is established between two user agents a media delivery protocol is used to transfer the media among the users. In particular, most of the SIP-based VoIP systems use the Real-time Transport Protocol~\cite{rfc3550} (RTP) to exchange  audio data, and use the Real-Time Transport Control Protocol~\cite{rfc3550} (RTCP) protocol to control the established RTP connections. User agents in SIP-based VoIP system are allowed to use an encryption-enabled version of RTP, called  Secure Real-time Transport Protocol~\cite{rfc3711} (SRTP), in order to secure their VoIP calls. Note that the encryption supported by SRTP is done end-to-end and the VoIP servers are not required to support encryption. We mandate the SIP-based design of \name to use SRTP for media transfer.

Similar to the case of Skype, if a user agent is behind a NAT or a firewall it will use an intermediate node to establish its VoIP connections.
%~\footnote{\url{http://sarp.sourceforge.net/}}\footnote{\url{http://www.rtpproxy.org/}}. 
%In particular, \amc{use of STUN and ICE??}. 
In particular, two popular techniques used by VoIP service providers to bypass NAT and firewalls are  \emph{session border controller} (SBC) \cite{sbc} and \emph{RTP bridge server}s \cite{sip-nat}. 
As in the case of the Skype-based \name, putting a \name server behind a firewall masks its IP address from censors, as the VoIP calls to it will be relayed through oblivious intermediate nodes.



%\amc{the generation of voip IDs for the server for different systems}

%\amc{security/privacy implications}


%\subsection{Other VoIP protocols}


